Synthetic Question Value Estimation for Domain Adaptation of Question Answering

Synthesizing QA pairs with a question generator (QG) on the target domain has become a popular approach for domain adaptation of question answering (QA) models. Since synthetic questions are often noisy in practice, existing work adapts scores from a pretrained QA (or QG) model as criteria to select high-quality questions. However, these scores do not directly serve the ultimate goal of improving QA performance on the target domain. In this paper, we introduce a novel idea of training a question value estimator (QVE) that directly estimates the usefulness of synthetic questions for improving the target-domain QA performance. By conducting comprehensive experiments, we show that the synthetic questions selected by QVE can help achieve better target-domain QA performance, in comparison with existing techniques. We additionally show that by using such questions and only around 15% of the human annotations on the target domain, we can achieve comparable performance to the fully-supervised baselines.

==> 1_Introduction.tex <==

\section{Introduction}
Question answering (QA) systems based on pretrained language models such as BERT \cite{Devlin19Bert} have recently achieved promising performance in machine reading comprehension.
However, neural QA systems trained on one domain may not generalize well to another, leaving it challenging to deploy such systems on new domains that lack large-scale QA training data\footnote{Large-scale training data are typically 60-100K in size.}. In this paper, we are interested in \emph{semi-supervised domain adaptation}: we aim to build a target QA model with source domain data and a small number of target annotated QA pairs.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/domain-adap-QA-intro.pdf}
    \caption{Existing work repurposes a pretrained QA (or QG) model to evaluate the quality of the generated questions, which is not directly associated with the target-domain QA performance. In contrast, our Question Value Estimator learns \emph{explicitly} to select the most useful questions for improving target-domain QA.}
    \vspace{-10pt}
    \label{fig:intro}
\end{figure}

Due to high annotation costs, existing work \cite{GolubHHD17,li2019Unified,WangGLLGW19,PuriSSPC20Training,chen20improved,yue2021contrastive} proposes to synthesize target-domain QA pairs via neural question generation (QG) models. The synthetic data are then used to train a QA model on the target domain. 
While the idea is attractive, in practice, the generated questions are of low quality, such as being semantically mismatched with their paired answers or asking about simple facts.
% (as shown in Section~\ref{?}). 
% For example, \citet{liu2020asking} show that a significant portion of questions generated by neural QG models are not well-formed or semantically mismatched with their paired answers. Moreover, many synthetic questions simply ask about trivial facts or are expressed in a trivial way (as shown in Section~\ref{?}). 
Including all such questions for QA training is less likely to bring substantial improvements. 
This inspires us to study a crucial problem:

% \begin{displayquote}
% Given a set of synthetic {question-answer pairs}, how to select high-quality ones that are semantically matched, non-trivial, and thus useful for the downstream QA model training?
% \end{displayquote}
\vspace{1pt}
\textit{Given a set of target-domain synthetic QA pairs, how to select high-quality ones that are useful to improve target QA training?}
\vspace{1pt}


To address the problem, \citet{Alberti19Synthetic} propose the Roundtrip Consistency filtering method, {which filters\footnote{We interchangeably use ``filter'' (noisy questions) and ``select'' (useful questions).} questions that cannot be correctly answered by a pretrained QA model}. Other work \cite{ShakeriSZNNWNX20} considers using the generation log likelihood by the QG model as a metric to filter noisy questions (Figure~\ref{fig:intro}, top).
Although these filtering techniques have been shown to improve the question quality to some extent \cite{RennieMMNG20}, they are not specifically designed to select questions \emph{that can improve QA performance on the target domain}. For example, some useful but difficult questions may be filtered by the Roundtrip method, since these questions cannot be answered correctly by the pretrained QA model. However, these questions are often crucial to further improving the QA performance when added into training.


In this paper, we propose to select synthetic questions with a novel \emph{question value estimator (QVE)} (Figure~\ref{fig:intro}, bottom). 
The QVE model has a transformer architecture (e.g., BERT) as the backbone. It takes in generated questions and their associated contexts and answers, and outputs real-valued scores (i.e., the question values) implying their usefulness for training a target-domain QA model. Based on the estimated question values, we can select useful ones from all the synthetic questions to train a target-QA model. Due to the lack of supervision (i.e., true question values), however, training the QVE model is challenging.
Intuitive solutions could be formulating QVE as either a binary classifier or a ranker over available human-annotated (positive or preferable) and machine-synthesized samples (negative or undesirable).
However, these baselines do not directly optimize QVE towards the goal of selecting useful synthetic QA pairs for improving the target QA performance.


To train QVE towards this goal, we formulate the question selection process of QVE as a reinforcement learning~\cite{Williams92} problem, and reward the model based on the direct feedback from the target QA. Specifically, the QVE model receives a batch of synthetic QA pairs each time and learns to select high-quality ones based on their estimated values. The select synthetic pairs are then used to train the downstream target-domain QA model, with the resulting performance gain (on the available target annotated QA pairs) used to determine whether the QVE model makes a good batch selection (i.e., assigns the question value properly for each example in the batch).

% To train QVE towards this goal, we formulate the question selection process of QVE as batch-level decision making. In each decision, the QVE model receives a batch of synthetic QA pairs and learns to select high-quality ones based on their estimated values. The select synthetic pairs are then used to train the downstream target-domain QA model, with the resulting performance gain (on the available target annotated QA pairs) used to determine whether the QVE model makes a good batch selection (i.e., assigns the question value properly for each example in the batch). Given the discrete question selection process, we train the QVE model using reinforcement learning~\cite{Williams92}, and reward the model by the performance gain it brings.


{To evaluate the QVE model, we instantiate the QG and the QA model based on the pretrained BART~\cite{Lewis20BART} and BERT~\cite{Devlin19Bert}, respectively.}
\textit{First}, by carrying out comprehensive experiments on four commonly-used reading comprehension datasets \cite{TrischlerWYHSBS17,JoshiCWZ17,Yang0ZBCSM18,KwiatkowskiPRCP19}, we show that our QVE model substantially outperforms existing filtering techniques. \textit{Second}, we show that QA models can achieve comparable performance to fully-supervised baselines when using QVE-selected synthetic questions plus around 15\% of the total target-domain training data.
\textit{Finally}, we conduct human evaluations and demonstrate that, when compared to existing filtering techniques, QVE can better identify semantically matched and more difficult questions, which explains the superior improvement it brings to the downstream QA task.





==> Tables/TableA2.tex <==
\begin{table}[t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|l|ccc}
\hline
Domain & Dataset & \#Train & \#Dev & \#Test \\ \hline
Source & SQuAD & 86,588 & 10,507 & - \\ \hline
\multirow{4}{*}{Target} & NewsQA & 74,160 & 1,000 & 4,212 \\
 & NQ & 104,071 & 1,000 & 12,836 \\
 & HotpotQA & 72,928 & 1,000 & 5,904 \\
 & TriviaQA & 61,688 & 1,000 & 7,785 \\ \hline
\end{tabular}
}
\caption{Statistics of the datasets. The numbers refer to the \#QA pairs (except the target-domain training sets where numbers refer to \#contexts). 1,000 annotated QA pairs are sampled as the target dev sets.}
\label{tbl:dataset}
\end{table}


==> Tables/table1.tex <==
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cl|cc|cc|cc|cc}
\hline
 \multirow{2}{*}{Settings} & \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{NewsQA} & \multicolumn{2}{c|}{NQ} & \multicolumn{2}{c|}{HotpotQA} & \multicolumn{2}{c}{TriviaQA} \\ \cline{3-10} 
 &  & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\ \hline
  & SynNet \cite{golub2017two} & 33.00 & 46.60 &-  &-  &-  &-  &-  &- \\
  & AdaMRC \cite{wang2019adversarial} & 38.46 & 54.20  &-  &-  &-  &-  &-  &- \\ 
  & UDA \cite{NishidaNSAT20}  &35.90  &51.40  &43.80  &56.70  &-  &-  &-  &- \\ \hline
%   & Info-HCVAE \cite{LeeLJKH20}   &-  &-  &48.44  &62.69  &-  &-  &50.14  &59.21 \\ \hline

% optional: trained on SQuAD 2.0
%   & \cite{MaharanaB20} &37.44  &48.95  &-  &-  &-  &-  &33.68  &40.99\\\hline
 
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Synthetic \\ Only\end{tabular}} & Fully-Synthetic Data   &  39.20&54.37  &  &  &  &  &00.00  &00.00 \\
 & +RoundTrip Filtering \cite{Alberti19Synthetic} &   40.57&54.64   &  &  &  &  &  & \\
 & +LM Filtering \cite{ShakeriSZNNWNX20} &  &  &  &  &  &  &  & \\
 & \textbf{+QVE (Ours)} &  &  &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Source  \\ + Synthetic \end{tabular}} 
& Source Only  &40.01  &55.34  &45.16  &59.12  &43.31  &60.32  &49.53  &59.28  \\
& +Fully-Synthetic Data  &40.38  &56.13  &54.81  &66.43  &46.17  &60.79  &54.02  &59.57  \\
 & +RoundTrip filtering \cite{Alberti19Synthetic} &43.61  &58.89  &  52.94 & 66.10   &45.77  &60.80  &58.84  &65.73 \\
  & +LM Filtering \cite{ShakeriSZNNWNX20} &  &  &  &  &  &  &  &  \\
 & \textbf{+QVE (Ours)} & \textbf{44.31}  &\textbf{59.89}  &\textbf{57.39}  &\textbf{69.66}  &\textbf{49.23}  &\textbf{64.82}  &\textbf{60.53}  & \textbf{66.67}
 \\\hline
  
 & Supervised target domain &   &   &  &  &00.00 & 00.00 &  &  \\\hline
\end{tabular}}
\caption{Overall domain adaptation performance of different models. The best performing method on each setting is in bold.}
\label{tbl:overall_performance}
\end{table*}

==> Tables/table1_5.tex <==
\begin{table*}[t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|l|cc|cc|cc|cc}
\hline
\multirow{2}{*}{Training Data} & \multirow{2}{*}{Row} & \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{NewsQA} & \multicolumn{2}{c|}{NQ} & \multicolumn{2}{c|}{HotpotQA} & \multicolumn{2}{c}{TriviaQA} \\ \cline{4-11} 
 & & & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\ \hline
   \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Wikipedia\end{tabular}} & 1& UnsupervisedQA\cite{LewisDR19}  & 17.5 & 25.6 &16.8  &24.9  &15.4  &23.3  &21.2  &27.5 \\
    & 2& RefQA\cite{li2020harvesting}\ACK  & 32.1 & 45.1 &- &- &-  &-  &-  &-\\\hdashline
   \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SQuAD + \\ Target Synthetic \, \end{tabular}}  &3 & UDA\cite{NishidaNSAT20}\ACK  &35.9  &51.4  &43.8  &56.7  &-  &-  &-  &- \\ 
  &4& SynNet \cite{GolubHHD17}\ACK  & 33.0 & 46.6 &-  &-  &-  &-  &-  &- \\
    &5& AdaMRC \cite{WangGLLGW19}\ACK  & 42.6 & 59.3  &-  &-  &-  &-  &-  &- \\ 
   &6&  Info-HCVAE \cite{LeeLJKH20}\ACK  &-  &-  &48.4  &62.7  &-  &-  &50.1  &59.2 \\ 
   &7&  CAQA \cite{yue2021contrastive}\ACK  &-  &-  &48.6  &62.6  &46.4  &61.6  &55.2  &63.2 \\ 
   \hline\hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Target \\ Synthetic\end{tabular}}  & 7 & Our QG Baseline & 41.9 & 56.3 & 54.8 & 67.1 & 43.5 & 58.2 & 50.8 & 59.5 \\
 & 8 & +RoundTrip Filtering \cite{Alberti19Synthetic} & 43.7 & 56.4 & 54.1 & 66.1 & 43.2 & 57.6 & 50.5 & 59.5 \\
 & 9 & +LM Filtering \cite{ShakeriSZNNWNX20} & 40.9 & 55.5 & 52.9 & 65.6 & 40.9 & 55.3 & 49.2 & 58.9 \\
 & 10 & +QVE (binary classifier) & 39.8 & 54.3 & 50.8 & 62.6 & 38.6 & 53.0 & 50.1 & 59.1 \\
 & 11 & +QVE (ranking baseline) & 40.5 & 55.2 & 54.2 & 67.0 & 40.5 & 55.1 & 51.2 & 59.9 \\
 & 12 & \textbf{+QVE (RL)} & \textbf{43.9} & \textbf{56.9} & \textbf{55.1} & \textbf{67.9} & \textbf{43.7} & \textbf{58.5} & \textbf{51.9} & \textbf{60.5} \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}SQuAD + \\ Target Synthetic \, \end{tabular}} & 13 & Our QG Baseline & 43.2 & 59.6 & 55.5 & 68.0 & 47.3 & 62.5 & 56.8 & 62.1 \\
 & 14 & +RoundTrip Filtering \cite{Alberti19Synthetic} & 44.4 & 60.2 & 57.3 & 69.0 & 49.0 & 64.8 & 58.6 & 63.2 \\
 & 15 & +LM Filtering \cite{ShakeriSZNNWNX20} & 44.2 & 60.1 & 54.0 & 67.7 & 48.1 & 63.2 & 58.4 & 63.1 \\
 & 16 & +QVE (binary classifier) & 42.0 & 58.7 & 52.8 & 65.6 & 45.5 & 60.5 & 56.4 & 61.2 \\
 & 17 & +QVE (ranking baseline) & 42.6 & 59.2 & 55.8 & 68.6 & 46.2 & 61.9 & 57.5 & 62.2 \\
 & 18 & \textbf{+QVE (RL)} & \textbf{44.6} & \textbf{60.4} & \textbf{57.8} & \textbf{69.7} & \textbf{49.7} & \textbf{65.2} & \textbf{59.3} & \textbf{63.7} \\ \hline
\end{tabular}%
}
\caption{Unsupervised domain adaptation performance. \ACK: Results are copied from the original paper and they may use a different data split from ours. The best performing method is in \textbf{bold}.}
\label{tbl:unsupervised_performance}
\end{table*}

==> Tables/table1_v2.tex <==
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lc|cccccccc}
\hline
 \multirow{2}{*}{Methods} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}QA Training\\ Data\end{tabular}}  & 
 \multicolumn{2}{c}{NewsQA} & \multicolumn{2}{c}{NQ} & \multicolumn{2}{c}{HotpotQA} & \multicolumn{2}{c}{TriviaQA} \\ \cline{3-10} 
  & & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\ \hline
   SynNet \cite{golub2017two} &SQuAD+Synth. & 33.0 & 46.6 &-  &-  &-  &-  &-  &- \\\hdashline
   AdaMRC \cite{wang2019adversarial}&SQuAD+Synth.  & 38.46 & 54.20  &-  &-  &-  &-  &-  &- \\ \hdashline
   Base\cite{NishidaNSAT20} &SQuAD  &35.2  &50.7  &44.4  &57.5  &-  &-  &-  &- \\ 
   UDA\cite{NishidaNSAT20}&SQuAD  &35.9  &51.4  &43.8  &56.7  &-  &-  &-  &- \\ \hline\hline
%   & Info-HCVAE \cite{LeeLJKH20}   &-  &-  &48.44  &62.69  &-  &-  &50.14  &59.21 \\ \hline

% optional: trained on SQuAD 2.0
%   & \cite{MaharanaB20} &37.44  &48.95  &-  &-  &-  &-  &33.68  &40.99\\\hline
 Source Only & SQuAD &40.01  &55.34  &44.68  &58.94  &43.31  &60.32  &49.53  &59.28  \\ \hline
 \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Our QG Baseline\end{tabular}} & Synthetic  &  38.03 & 52.83  &  &  &  &  &  & \\
  &SQuAD+Synth. &39.15  &55.40  &54.81  &66.43  &46.17  &60.79  &54.02  &59.57  \\ \hdashline
 
 \multirow{2}{*}{\quad\begin{tabular}[l]{@{}l@{}}+RoundTrip Filtering\\\cite{Alberti19Synthetic}\end{tabular}}  &Synthetic &40.57 &54.64   &  &  &  &  &  & \\
 &SQuAD+Synth. &43.61  &58.89  &  52.94 & 66.10   &45.77  &60.80  &58.84  &65.73 \\ \hdashline

 \multirow{2}{*}{\quad\begin{tabular}[l]{@{}l@{}}+LM Filtering\\\cite{ShakeriSZNNWNX20}\end{tabular}}  &Synthetic &  &  &  &  &  &  &  & \\
  &SQuAD+Synth. &  &  &  &  &  &  &  &  \\\hdashline
 
\textbf{\multirow{2}{*}{\quad+QVE (Ours)}} &Synthetic &  &  &  &  &  &  &  &  \\ 
 &SQuAD+Synth. & \textbf{44.31}  &\textbf{59.89}  &\textbf{57.39}  &\textbf{69.66}  &\textbf{49.23}  &\textbf{64.82}  &\textbf{60.53}  & \textbf{66.67}
 \\
 \hline\hline
  
  Supervised target domain &Target   &50.00   &64.61  &65.82  &78.06 &56.82  &73.89  & 64.58 & 70.28 \\\hline
\end{tabular}}
\caption{Overall domain adaptation performance of different models. The best performing method on each setting is in bold.}
\label{tbl:overall_performance}
\end{table*}

==> Tables/table1_v3.tex <==
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|lc|cccccccc}
\hline
 \multirow{2}{*}{Row} &\multirow{2}{*}{Methods} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}QA Training\\ Data\end{tabular}}  & 
 \multicolumn{2}{c}{NewsQA} & \multicolumn{2}{c}{NQ} & \multicolumn{2}{c}{HotpotQA} & \multicolumn{2}{c}{TriviaQA} \\ \cline{4-11} 
  & & & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\ \hline
  1& \cite{LewisDR19} &Wikipedia & 17.5 & 25.6 &16.8  &24.9  &15.4  &23.3  &21.2  &27.5 \\\hdashline
   2&   Base\cite{NishidaNSAT20}\ACK &SQuAD  &35.2  &50.7  &44.4  &57.5  &-  &-  &-  &- \\ 
   3& UDA\cite{NishidaNSAT20}\ACK&SQuAD+Target Contexts  &35.9  &51.4  &43.8  &56.7  &-  &-  &-  &- \\ \hdashline
   4& SynNet \cite{GolubHHD17}\ACK &SQuAD+Target Gen QAs & 33.0 & 46.6 &-  &-  &-  &-  &-  &- \\
   5& AdaMRC \cite{WangGLLGW19}\ACK&SQuAD+Target Gen QAs  & 42.6 & 59.3  &-  &-  &-  &-  &-  &- \\ 
   6&  Info-HCVAE \cite{LeeLJKH20}\ACK & SQuAD+Target Gen QAs &-  &-  &48.4  &62.7  &-  &-  &50.1  &59.2 \\ 
   \hline\hline

 7& Our Source Only Baseline & SQuAD &40.2	&56.2	&45.2	&59.1	&43.3	&60.3	&49.5	&59.3  \\ \hline
 8& \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Our QG Baseline\end{tabular}} & Target Gen QAs  &{41.9}	&{56.3}	&54.8	&67.1	&43.5	&58.2	&57.4	&62.4 \\
 9 & &SQuAD+Target Gen QAs &43.2	&59.6	&55.5	&68.0	&47.3	&62.5	&59.7	&64.8  \\ \hdashline
 
 10& \multirow{2}{*}{\quad\begin{tabular}[l]{@{}l@{}}+RoundTrip Filtering\\\cite{Alberti19Synthetic}\end{tabular}}  &Target Gen QAs &41.7	&55.3	&52.9	&65.6	&42.0	&56.6	&56.0	&62.6 \\
 11& &SQuAD+Target Gen QAs &{44.8}	&{60.1}	&54.0	&67.4	&47.4	&62.5	&60.3	&67.2 \\ \hdashline

 12& \multirow{2}{*}{\quad\begin{tabular}[l]{@{}l@{}}+LM Filtering\\\cite{ShakeriSZNNWNX20}\end{tabular}}  &Target Gen QAs &40.9	&55.5	&52.9	&65.6	&40.9	&55.3	&53.5	&58.9 \\
 13&  &SQuAD+Target Gen QAs &44.2	&60.1	&54.0	&67.7	&48.1	&63.2	&58.4	&64.1  \\\hdashline
 
14& \textbf{\multirow{2}{*}{\quad+QVE (Ours)}} &Target Gen QAs &{\textbf{44.2}}	&{\textbf{60.0}}	&{\textbf{55.2}}	&{\textbf{67.6}}	&{\textbf{44.9}}	&{\textbf{60.0}}	&{\textbf{57.6}}	&{\textbf{62.9}}  \\ 
15&  &SQuAD+Target Gen QAs &{\textbf{46.3}}	&{\textbf{61.8}}	&{\textbf{57.6}}	&{\textbf{69.9}}	&{\textbf{50.5}}	&{\textbf{66.2}}	&{\textbf{62.0}}	&{\textbf{67.7}}
 \\
 \hline\hline
  
 16&  Supervised target domain &Target   &50.0	&64.6	&65.8	&78.1	&56.8	&73.9	&64.6	&70.3 \\\hline
\end{tabular}}
\caption{Overall domain adaptation performance of different models. \ACK: Results are copied from the original paper and ``-" means results are not reported in the original paper. The best performing method is in \textbf{bold}.}
\label{tbl:overall_performance}
\vspace{-15pt}
\end{table*}

==> Tables/table2.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|c|c}
\hline
Datasets & Method & EM & F1 \\ \hline
   \multirow{4}{*}{NewsQA} & QG Baseline  &43.2  &59.6  \\ 
   &\,+ Finetuned QG w/ QAP &44.4  &60.8  \\
 &\,\textbf{+ Finetuned QG w/ QVE (Ours)} &\textbf{45.8}  &\textbf{61.2}  \\
 &\quad \textbf{+ QVE filtering (Ours)} &\textbf{47.2}  &\textbf{62.9}  \\
 \hline 
    \multirow{4}{*}{NQ} & QG Baseline  &55.5   &68.0  \\ 
   &\,+ Finetuned QG w/ QAP &58.1  &69.3  \\
 &\,\textbf{+ Finetuned QG w/ QVE (Ours)} &\textbf{59.2}  &\textbf{70.3}  \\
 &\quad \textbf{+ QVE filtering (Ours)} & \textbf{60.1} & \textbf{71.8}  \\
 \hline 
    \multirow{4}{*}{HotpotQA} & QG Baseline  &47.3   &62.5  \\ 
   &\,+ Finetuned QG w/ QAP & 49.2 & 64.2 \\
 &\,\textbf{+ Finetuned QG w/ QVE (Ours)} & \textbf{49.9}  & \textbf{65.3}  \\
 &\quad \textbf{+ QVE filtering (Ours)} &\textbf{51.3}  &\textbf{67.3}  \\
 \hline 
    \multirow{4}{*}{TriviaQA} & QG Baseline  & 59.7  & 64.8  \\ 
   &\,+ Finetuned QG w/ QAP & 60.8  & 65.2 \\
 &\,\textbf{+ Finetuned QG w/ QVE (Ours)} & \textbf{61.5} & \textbf{66.7}  \\
 &\quad \textbf{+ QVE filtering (Ours)} &\textbf{63.3}  &\textbf{68.9}  \\
 \hline 
\end{tabular}}%
\caption{QA performance based on finetuned QG models (with different training signals). \add{to be updated...}}
\label{tbl:finetuned-qg}
\end{table}









%%%%%%%%%%%%OLD RESULTS

% Datasets & Method & EM & F1 \\ \hline
%   \multirow{2}{*}{NewsQA} & QG Baseline  &   &  \\ 
%   &\,+ Finetuned QG w/ QAP &  &  \\
%  \hline  \hline
%   \multirow{2}{*}{NQ}  & QG Baseline + QVE & 57.39  & 69.66 \\ 
%  &\quad + Finetuned QG + QVE &\textbf{59.63}  &\textbf{71.65}  \\
%  \hline  \hline
%  \multirow{2}{*}{HotpotQA} 
%  & QG Baseline + QVE & 49.23  & 64.82 \\ 
%  &\quad + Finetuned QG + QVE &\textbf{50.53}  & \textbf{65.86}  \\
%  \hline  \hline
%  \multirow{2}{*}{TriviaQA} 
%  & QG Baseline + QVE & 60.53  & 66.67 \\ 
%  &\quad + Finetuned QG + QVE &\textbf{62.19}  & \textbf{67.67} \\

==> Tables/table4.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ccc}
\hline
Iteration & \textbf{NQ} & \textbf{HotpotQA}  \\ \hline
0  & 48.11/53.22 & 48.11/53.22\\
1 & \textbf{48.11/53.22} & \textbf{48.11/53.22}\\
2  & 48.11/53.22 & 48.11/53.22 \\
3  & 48.11/53.22 & 48.11/53.22 \\
\hline
\end{tabular}
\caption{Results of finetuning the framework with multiple iterations}
\label{tbl:multi-iterations}
\end{table}

